B-cos GNNs: Faithful Explanations through Dynamic Linearity

We introduce B-cos GNNs, an inherently explainable class of graph neural networks whose predictions decompose exactly into per-node, per-feature contributions via a single input-dependent linear map. B-cos GNNs use linear (sum-based) aggregation and replace non-linear message and update functions with B-cos transforms. This induces meaningful, task-specific weight-input alignment that is directly accessible through the model's dynamic linearity. Instance-level explanations follow from a single forward and backward pass, requiring no auxiliary explainer, modified learning objective, or perturbation procedure. Instantiated as a GIN, our approach trades small losses in predictive accuracy for state-of-the-art explainability across diverse synthetic and real-world benchmarks, producing explanations orders of magnitude faster than post-hoc baselines.

==> b_sensitivity_table.tex <==
\begin{table}[ht]
    \begin{tabular}{l|cccc|cccc}
    \toprule
     & \multicolumn{4}{c|}{\textbf{BA-2Motif}} & \multicolumn{4}{c}{\textbf{Di-Halo-Benzene}} \\
    \textbf{Param} & \textbf{Acc} & \textbf{Jacc.} & \textbf{AUC} & \textbf{Total (s)} & \textbf{Acc} & \textbf{Jacc.} & \textbf{AUC} & \textbf{Total (s)} \\
    \midrule
    $B=1.0$ & 0.726 & 0.15{\scriptsize$\pm$0.01} & 0.47{\scriptsize$\pm$0.00} & \textbf{9.2{\scriptsize$\pm$0.1}} & 1.000 & 0.57{\scriptsize$\pm$0.05} & 0.91{\scriptsize$\pm$0.03} & 118.2{\scriptsize$\pm$15.1} \\
    $B=1.5$ & \textbf{1.000} & 0.81{\scriptsize$\pm$0.02} & 0.91{\scriptsize$\pm$0.02} & 17.9{\scriptsize$\pm$0.1} & \textbf{1.000} & 0.91{\scriptsize$\pm$0.06} & 0.99{\scriptsize$\pm$0.01} & 122.2{\scriptsize$\pm$4.3} \\
    $B=2.0$ & \textbf{1.000} & 0.84{\scriptsize$\pm$0.05} & 0.94{\scriptsize$\pm$0.05} & 16.6{\scriptsize$\pm$0.9} & \textbf{1.000} & \textbf{0.94{\scriptsize$\pm$0.06}} & 0.97{\scriptsize$\pm$0.05} & \textbf{88.6{\scriptsize$\pm$9.1}} \\
    $B=2.5$ & \textbf{1.000} & 0.87{\scriptsize$\pm$0.05} & 0.98{\scriptsize$\pm$0.02} & 21.5{\scriptsize$\pm$0.8} & \textbf{1.000} & 0.93{\scriptsize$\pm$0.03} & \textbf{0.99{\scriptsize$\pm$0.01}} & 131.6{\scriptsize$\pm$23.8} \\
    $B=3.0$ & \textbf{1.000} & \textbf{0.89{\scriptsize$\pm$0.05}} & \textbf{0.99{\scriptsize$\pm$0.00}} & 18.5{\scriptsize$\pm$0.5} & \textbf{1.000} & 0.86{\scriptsize$\pm$0.07} & 0.98{\scriptsize$\pm$0.01} & 124.1{\scriptsize$\pm$33.6} \\
    \bottomrule
    \end{tabular}
    \label{tab:b_sensitivity}
\end{table}
